Adaptive Reduced Rank Regression

We study the low rank regression problem $\my = M\mx + \epsilon$, where $\mx$ and $\my$ are $d_1$ and $d_2$ dimensional vectors respectively. We consider the extreme high-dimensional setting where the number of observations $n$ is less than $d_1 + d_2$. Existing algorithms are designed for settings where $n$ is typically as large as $\Rank(M)(d_1+d_2)$. This work provides an efficient algorithm which only involves two SVD, and establishes statistical guarantees on its performance. The algorithm decouples the problem by first estimating the precision matrix of the features, and then solving the matrix denoising problem. To complement the upper bound, we introduce new techniques for establishing lower bounds on the performance of any algorithm for this problem. Our preliminary experiments confirm that our algorithm often out-performs existing baselines, and is always at least competitive.

==> exp_tweet.tex <==
\subsubsection{Social network data set}\label{dataset_twitter}
This section demonstrates the effectiveness of our algorithm in Twitter dataset. 
%We aim to forecast users' popularity in time series. Predict the users' popularity has profound impact in social media since it reveals the public attention and is a strong indicator of online marketing. 
Our goal is to predict a user's \emph{next 1-day} popularity, which is defined as the sum of retweets, quotes, and replies received by the user.  We focus on tweets with topics related to politics. User's popularity is more or less influenced by the other users since they might have collaboration or competition relationship. It suggests that features from the other users can be used to boost the prediction. To benefit from these shared features and improve the generalization performance, we cast the predicting problem as multi-variate regression  where we make users' future popularity predictions based on the features from all the users. However, it is challenging to consume such a large number of features.  The feature size is much larger than the number of observations which is more likely to end up with overfitting issues. 
Moreover, the dynamical nature of social networks and user diversity lead to a high noise-to-signal ratio in the social network dataset and make the prediction more difficult.


\myparab{Measure the user popularity}
We highlight three types of interactions on Twitter to measure the user's popularity.
First, users directly comment on another person’s tweet. The action is called reply and the number of replies indicates audience activeness for that user. 
Second, users repost another person's tweet to their followers. This action is called retweet. The number of retweets indicates the user's ability to generating popular contents. Finally, the users quote/mention another person’s username anywhere in the body of the tweet. The number of quotes/mentions indicates the ability of that user to engage others in a conversation. 


\myparab{Tweeter dataset collection}
We collected 15 months Twitter data from October 01, 2016 to December 31, 2017, using the Twitter streaming API. We tracked the tweets with topics related to politics with keywords ``trump”, ``clinton”, ``kaine”, ``pence”, and ``election2016”. There are a total of 804 million tweets and 19 million distinct users. User $u$ has one interaction if and only if he or she is retweeted/replied/quoted by another user $v$. We followed the data preprocessing in~\cite{li2017world}. There are a total of 19 million distinct users, and due to the huge size, we extract the subset of 2000 users with the most interactions for evaluation.
We use the period from October 01, 2016 to June 30, 2017 as the training dataset, the period from July 01, 2017 to October 30 as validation dataset to optimize the hyper-parameters, and the rest of the period, from September 10, 2017 to December 31, 2017, is used for the performance evaluation. 




\myparab{Problem formatting}
Our goal is to forecast the  \emph{next 1-day} users popularity based on 
 \emph{all users' past popularity}. Let $y_{i, t}$ be the popularity for user $i$ at time $t$ and there are $d_2$ users to forecast, then $\my_{t} = (y_{i,t}:i \leq d_2)$. 
We tackle the problem by casting it as an inference problem of $\my_{t+1} = M \mx_t + \epsilon$, where $\mx_{t} \in \reals^{d_1}$, $\my_{t+1} \in \reals^{d_2}$, $M\in\reals^{d_2\times d_1}$. We denote $\mx_{t} $ as popularity features form all the users at time $t$ and we aim to forecast users' \emph{next 1-day} popularity $\my_{t+1}$.
%We construct $\mx$ and $\my$ from the training traces to solve for $M$. Then we plug in the estimated $M$ and construct $\mx$ from the testing traces to predict $\my$ for the testing trace.

\myparab{Features and response}
For each user in the universe, we compute their past $k_1$ days popularity as the features. We set $k_1 = 5$ in our experiment.  There are 2000 users, therefore the total number of features is $d_1 = 2000k_1$.
Since there are 240 observations in the training data set, to 
followed our assumption where $d_1 >> n $ and $d_2$ has similar magnitude towards $n$, we randomly sample 200 users from the universe to make forecast on these users and $d_2 = 200$. 

\iffalse

\myparab{Characteristic}
We illustrate the statistics from Twitter dataset in Figure~\ref{fig:characteristic}.
Figure ~\ref{fig:characteristic}(a) shows the log log plot of eigenvalues for feature covariance matrix from the training period. It exhibits the power law distribution for the feature covariance matrix. 
The Figure~\ref{fig:characteristic}(b) illustrates the gap between two consecutive eigenvalues of covariance matrix in log scale. 
%Figure~\ref{fig:characteristic}(c) shows the distribution for users' average daily activeness. 
 
\begin{figure}[h!]
    \centering
    \begin{minipage}[h]{0.45\linewidth}
        \center{\includegraphics[width=1\linewidth]{figures/tweet_loglog.pdf}} \small{a) Log log plot of eigenvalues}
        \label{hist_sum_user}
    \end{minipage}
    \begin{minipage}[h]{0.45\linewidth}
        \center{\includegraphics[width=1\linewidth]{figures/log_gap.pdf}} \small{b) Log of gap in eigenvalues} 
        \label{std_user}
    \end{minipage}
    \caption{Statistics from Twitter dataset.}
    \label{fig:characteristic}
\end{figure}
\fi

\myparab{Results} 
The training period has 240 observations, validation period has 60 observations and testing dataset consists of 100 observations. Note that one observation is a $(\mx_t,\my_t)$ pair. 
%We report the forecasting power for both \emph{in-sample} and \emph{out-of-sample} periods. 
We randomly sample the users for 10 times and report the MSE and correlation with their standard deviation for both \emph{in-sample} and \emph{out-of-sample} in the Table~\ref{table:tweets_app}. We can see consistent results similar to the equity return forecast where \emph{(i)}
Our model yields the best performance in terms of MSE and correlation compared to other baselines, demonstrating the effectiveness of our algorithm on high-dimensional and high noise-to-signal data set. \emph{(ii)} Better %generation
generalization
guarantees. Our model achieves a much smaller gap between training and testing errors than the other baselines.







\begin{table}[h!]
\centering
\begin{tabular}{l|l|l|l|l|l}
\hline
Models    & MSE$_{in}$ & MSE$_{out}$ & MSE$_{out-in}$ & Corr$_{in}$ & Corr$_{out}$        \\ \hline
$\proc{Adaptive-RRR}$      & 5.0104 $\pm$ {0.38}  &  \textbf{9.4276} $\pm$ 2.31 &  \textbf{4.4172}  & 0.7425 $\pm$ 0.07 & \textbf{0.6730} $\pm$ 0.13 \\
Lasso     & 2.3755  $\pm$ 1.95 & 14.8279 $\pm$ 4.81 & 12.4524 &  0.9171  $\pm$ 0.09 & 0.4754  $\pm$  0.15\\
Ridge     &1.3974 $\pm$ {0.53}  & 13.6244 $\pm$ 4.39 & 12.2270 & 0.9555  $\pm$ 0.04 & 0.4742 $\pm$ 0.17 \\
Reduced ridge & 4.5260 $\pm$ {1.93}  & 12.2339 $\pm$ 2.70  & 7.7079  & 0.7905 $\pm$ 0.09 & 0.4972 $\pm$ 0.18 \\
RRR       & 4.3456 $\pm$ {0.47} & 13.0768 $\pm$ 2.63 & 8.7313  & 0.7725 $\pm$ 0.12 & 0.3820 $\pm$ 0.22\\
Nuclear norm  & 4.9190 $\pm$ {2.04} & 13.0532 $\pm$ 4.38 & 8.6677 & 0.7872  $\pm$ 0.10 & 0.4869 $\pm$ 0.16\\
\hline
\end{tabular}
\caption{The average results for Twitter dataset from 10 random samples. Bold font denotes the best \emph{out-of-sample} results and smallest gap.}
\label{table:tweets_app}
\end{table}





==> full_exp.tex <==
\newpage
\onecolumn
\section{Full experimental results}\label{asec:exp}
\iffalse
\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.5\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/high_level_statement.pdf}
\caption{High level statement}
\label{high_level}
\end{subfigure}
\begin{subfigure}[b]{0.4\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/space_as_one.pdf}
\caption{Parameter space}
\label{para_space}
\end{subfigure}
\caption{Figures to use}
\label{fig:high_and_param}
\end{figure}
\fi


In this section, we describe our experimental results obtained from both synthetic and real datasets. 
\subsection{Synthetic data}\label{asec:syn}
We evaluate our algorithm on synthetic data to gain further insights into its theoretical properties.
We produce synthetic data using the linear model $\mY = \mX M^{\transpose} + E$. $\mX$ comes from a matrix of i.i.d.\ standard Gaussian random variables, whose covariance matrix's eigenvalues follow a power law distribution. To generate $M$, we first randomly sample entries from $\{-1,0,1\}$, and then we run SVD to construct a low rank approximation of it. 
Finally, $E$'s entries are i.i.d.\ $N(0, \sigma_{\text{noise}}^2)$ with $\sigma_{\it{noise}} = \eta \cdot \text{std}(\text{vec}(\mX M^{\transpose}))$ and $\eta$ is a noise multiplier parameter. 





\begin{figure}[h!]
\centering
\includegraphics[width=0.85\linewidth]{figures/k1k2_error_new1.pdf}
\caption{Reconstruction error $\|M-\hat{M}\|_F$ at different $(k_1,k_2)$ for varying noise levels. The dashed lines correspond to the true rank of $M$ and the `x' marks the $(k_1, k_2)$ with the lowest error.}
\label{fig:k1k2_errora}
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[width=0.85\linewidth]{figures/k1k2_mse_new1.pdf}
\caption{Out-of-sample MSE: $\|\mY_{\text{out}}-\mX_{\text{out}}\hat{M}^{\transpose}\|_F$.}
\label{fig:k1k2_msea}
\end{figure}
\begin{figure}
\centering
\includegraphics[width=0.85\linewidth]{figures/k1k2_corr_new1.pdf}
\caption{Out-of-sample correlation.}
\label{fig:k1k2_corra}
\end{figure}
\begin{figure}
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\linewidth]{figures/reconstruction_error_200.pdf}
\caption{Reconstruction error.}
\label{fig:varynoisea:error}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\linewidth]{figures/Rsquare_200.pdf}
\caption{Out-of-sample $R^2$.}
\label{fig:varynoisea:corr}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
\includegraphics[width=\linewidth]{figures/rank_200.pdf}
\caption{Recovered rank.}
\label{fig:varynoisea:rank}
\end{subfigure}
\caption{Algorithm comparison with varying noise multipliers $\eta$ and fixed $\text{rank}(M) = 10$. Error bars report 1 standard deviation from 50 runs.}
\label{fig:varynoisea}
%\vspace{-0.6cm}
\end{figure}

In the Figures.~\ref{fig:k1k2_errora},~\ref{fig:k1k2_msea} and \ref{fig:k1k2_corra}, we consider $\text{rank}(M) = 50$ and $d_1 = 200$, $d_2 = 100$ and $n = 150$ (similar results under other settings). We sweep the $(k_1, k_2)$ space and measure the reconstruction error on $M$ due to our algorithm in Figure.\ \ref{fig:pcarrr}. We observe that when the noise level is low ($\eta = 0.25$), the optimal $k_1$ can be much larger than $\text{rank}(M)$, while the optimal $k_2$ is $\text{rank}(M)$. This is consistent with our theoretical results.
However, as the noise level increases, the optimal $(k_1, k_2)$ shrinks to values smaller than $\text{rank}(M)$, which demonstrates the ability of our algorithm to adapt $\hat{M}$'s rank to signal-to-noise ratios. Figures.\ \ref{fig:k1k2_msea} and \ref{fig:k1k2_corra} show how our algorithm performs in terms of out-of-sample MSE and correlation on $\mX_{\text{out}}$ and $\mY_{\text{out}}$, which are generated in the same way as $\mX$ and $\mY$ under fixed $M$. The two metrics (commonly used in real applications) are qualitatively similar to reconstruction error (which is usually unobservable). 


We next compare our algorithm with other regularized regression methods, including ridge regression (``Ridge''), reduced rank ridge regression \cite{mukherjee2011reduced} (``Reduced ridge''), LASSO (``Lasso''), nuclear norm regularized regression (``Nuclear''), and reduced rank regression (``RRR''). We set $n=150$, $d_1 = 200$, $d_2=150$, rank$(M)=10$, and $\omega=2$. 
For each regression method, we sweep its regularization parameter(s) and report the best performance.  
Figures.\ \ref{fig:varynoisea:error} and \ref{fig:varynoisea:corr} show that our algorithm performs significantly better than other commonly used regularization strategies (ridge regression, LASSO, and nuclear norm regularization), and has similar performance as reduced rank ridge regression. Such observations echo our theoretical analysis well. Figure.\ \ref{fig:varynoisea:rank} shows the rank of $\hat{M}$ from the regression methods. Our algorithm, Reduced ridge, and RRR are able to adapt (reduce) the rank when the noise level is high, while Nuclear consistently attempts to recover the true rank of $M$, which sometimes leads to poor performance.

\qq{Do we still need the Table and paragraph below}
We also examine the in-sample and out-of-sample MSE in reduced rank regression (RRR) and fix $\eta = 0.4$. Table~\ref{tlb:app_rrr_mse_app} shows that even $k$ in RRR is very small, there is a huge gap between training and test error, which indicates severe overfitting problem. 

\begin{table}[h]
\centering
\vspace{-0.3cm}
\caption{In-sample and out-of-sample error on $\mY$ and $\mY_{out}$ for RRR ($\eta = 0.4$). }
\begin{tabular}{l|l|l|l|l|l}
\hline
               & $k$ = 1   & $k$ = 2   & $k$ = 3   & $k$ = 4    & $k$ = 5    \\ \hline
Training error & 0.3918 & 0.2813 & 0.2196 & 0.1952  & 0.1803  \\ \hline
Testing error & 5.8739 & 7.4833 & 8.7095 & 18.8408 & 19.3230 \\ \hline
\end{tabular}
\label{tlb:app_rrr_mse_app}
\vspace{-0.2cm}
\end{table}


\subsection{Real dataset}

Our method can be applied to many applications from various fields describing the real-world phenomena that their features spectrum follows a power-law distribution~\cite{konect:2017:flickr-links,akemann2010universal,konect:leskovec107,clauset2009power,konect:2017:facebook-wosn-links}. We apply our algorithm on an equity market and a social network dataset to predict equity returns and user popularity respectively.


\myparab{Distribution of eigenvalues.}
To justify the use of our algorithm, Figure~\ref{fig:characteristic_app} shows our datasets have feature covariance matrix eigenvalues decay at or faster than a power law distribution. We also verify the (upper bounding) power law distributions (as indicated by dotted lines) have $\omega > 2$.



\begin{figure}[h!]
\centering
\begin{subfigure}[b]{0.3\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/stock_loglog.pdf}
\caption{Equity market dataset}
\label{loglogE}
\end{subfigure}
\hspace{4em}
\begin{subfigure}[b]{0.31\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/Twitter_loglog.pdf}
\caption{Social network dataset.}
\label{loglogT}
\end{subfigure}
\caption{CDF of eigenvalues of feature covariance matrix.}
\label{fig:characteristic_app}
\end{figure}


\subsubsection{Equity markets}\label{asec:real}

First, we evaluate the performances of our forecasting methods for predicting equity returns. We use an emerging stock market. The data consists of approximately 3600 stocks between 2011 and 2018. We use the open (9:30 am) to open price to compute returns at daily frequency. The returns only cover regular trading days.
We examine two different universes in this market:
(i) \emph{Universe 1} is equivalent to the S$\&$P 500 and consists of 983 stocks \footnote{The universe usually consists of 800 stocks but it evolves slowly; 983 is the total number of stocks that appeared in the universe}, and (ii) \emph{Full universe} consists of all stocks except for illiquid ones.


\myparab{Responses.} We focus on predicting the \emph{next 5-day returns} for different universes. In this section, we take Table~\ref{table:800_equity} as an example. The universe includes 800 equities. Therefore $d_2 = 800$. The next-5-day forecast is produced for every trading day. Let $r_{i, t}$ be the return of the $i$-th asset for time interval $t$. Let $\mr_t = (r_{i, t}: i \leq d_2)$. 
%selected by market capitalization and trading volume. {\color{blue}not sure how selected  800} 

\iffalse
the ``largest'' 200 stocks (in terms of average dollar volume). Therefore $d_2 = 200$. The universe is selected at the end of each training period (\ie we determine the universe using the training data before training) so that there is no look-ahead or survival bias. The next-two-hour forecast is produced for every 5 minutes.
\fi

\myparab{Features.} For each asset in the universe, we compute its past 1-days, past-5 days and past 10-days returns as part of the feature. Therefore, the total number of features is $d_1 = 2400$. Let $\mx_t$ be the feature vector at time $t$. We remark that each feature has limited forecasting power (which is implicitly implied from LASSO). 


\myparab{Model, training, and hyper-parameters.} Our regression model is 
\begin{align}
\mr_{t+1} = M \mx_t + \epsilon. 
\end{align}
%We use a sliding window approach~\cite{chan2017machine} to train the model, using three year data for training. 
We use three year data for training, one year for validation and one year for testing. 
%We use validation set to tune the hyper-parameters. 
The model is re-trained every test year. 
For example, the training period is May 1, 2011 to May 1, 2014 and the validation period is from June 1, 2014 to June 1, 2015.
We use the validation set to determine the hyperparameters and build the model, and then we use the trained model to forecast returns of equity in the same universe from July 1, 2015 to July 1, 2016. Then the model is retrained by using data in the second training period (May 1, 2012 to May 1, 2015). This workflow repeats. To avoid the look-ahead issue, we set the gap between the training and validation set
as one month, which is the same as the gap between the validation and testing set.


 \myparab{Optimization.} We use standard approach to translate forecasts into positions~\cite{grinold2000active,prigent2007portfolio,ang2014asset,zhou2014active}. Roughly speaking, the position is proportional to the product of forecasts and a function of average dollar volume. We allow short-selling. We do not consider transaction cost and market impact. We do not hold overnight positions so the exposure to the market is minimum. 
%{\color{red} Check: 1. name of the models, 2. Ridge \& Adaptive is removed.}

\iffalse
\myparab{Results.}≈ We report the forecasting power and portfolio return for \emph{out-of-sample} periods. Because the forecasts are serially correlated (\eg at time 9:30 am, we will forecast the return between 9:30 and 11:30, and at 9:35 am, we will forecast between 9:35 and 11:35), we use Newey-West and non-parametric methods to estimate the $t$-statistics (see \eg~\cite{bickel1981some,greene2003econometric}).
We do not show returns' correlation with the market, because there is no overnight holding. 
%The average number of observations of training set and testing set are 11702 and 1964. 
\fi


\iffalse
\mypara{Obs 4. Orthogonal signals.} The signals we produce (our forecast $\hat \mr_t$) appear to be quite orthogonal to the rest of the models. For example, if we residualize our forecast against ridge model (second best model), we still have around 20bps forecasting power. 
\fi
%This section describes additional statistics on our equity dataset. 
\iffalse
\myparab{Distribution of the eigenvalues and gaps.}
Figure.~\ref{fig:Xtrain_statistic} (a) shows the distribution of the eigenvalues of the feature covariance matrix from training periods in \emph{Universe 1}. Their consistent behaviors are evidence of time series stationarity. It indeed exhibits decay and long-tail behaviors, and thus satisfies our assumption about power law decay (see Sec.~\ref{sec:prelim}). The tails are in general small, so it is necessary to cut out them to achieve improved performance (confirmed in experiments in Sec.~\ref{sec:exp}). Figure.~\ref{fig:Xtrain_statistic} (b) shows the gap between two consecutive eigenvalues of the covariance matrix in log scale. They all are non-monotonic, confirming the need to develop a theory using only the asymptotic decay assumptions (asymptotic decays allow non-monotonic gaps). 
\qq{Might be we should move out this section and the Figure 12?}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/xtrain_eig_figs.png}
    \caption{Statistics from eigenvalues of the feature covariance matrix and the x-axis is the training duration.}
    \label{fig:Xtrain_statistic}
\end{figure}
\fi
\iffalse
\begin{figure}[h!]
 \centering
 \iffalse
  \begin{subfigure}[b]{0.5\textwidth}
 \includegraphics[width=\linewidth]{figures/engivalues_Xtrain.png}
	 \caption{\small{Distribution of eigenvalues}}
 \end{subfigure}
 \fi
 \begin{subfigure}[b]{0.48\textwidth}
 \includegraphics[width=\linewidth]{figures/loglog.png}
	 \caption{\small{Log log plot of eigenvalues}}
 \end{subfigure}
  \begin{subfigure}[b]{0.48\textwidth}
 \includegraphics[width=\linewidth]{figures/log_gap.png}
	 \caption{\footnotesize{Log of gap in eigenvalues}}
 \end{subfigure}
 \caption{{\footnotesize Statistic from China stock and the x-axis is the training duration.
 }}
 \label{fig:Xtrain_statistic}
\end{figure}
\iffalse
\begin{figure}[h!]
 \centering
 \begin{subfigure}[b]{0.49\textwidth}
 \includegraphics[width=\linewidth]{figures/histogram_ypred.png}
	 \caption{\footnotesize{Histogram for sum of our prediction}}
 \end{subfigure}
 \begin{subfigure}[b]{0.49\textwidth}
 \includegraphics[width=\linewidth]{figures/std_preY.png}
	 \caption{\small{Standard deviation for our prediction}}
 \end{subfigure}
 \caption{{\footnotesize Statistic from our predicted returns on four randomly picked test sets. The x-axis is the testing duration.
 }}
 \fi
 
 %\vspace{-0.2cm}
 \label{fig:preY_statisticaa}
\end{figure}
\fi
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/hist_std_y.png}
    \caption{\footnotesize Statistics from our predicted returns on \emph{Universe 1}. The x-axis is the testing duration.}
    \label{fig:preY_statisticaa}
\end{figure}

 
\begin{table}[h]
\vspace{.2cm}
\begin{center}
\captionsetup{font= large}
%\captionsetup{justification=centering}
\caption{Data column names and their explanations}
    \begin{tabular}{  l|  p{9cm}}
    \hline
   \textbf{Column name}  & \textbf{Explanation} \\ \hline
Test start date & The start date of the testing period   \\
$N$ & The universe size  \\
MSE$_{out}$ & Normalized out-of-sample mean squared error (normalized by standard deviation of the responses) \\
MSE$_{in}$ & Normalized in-sample mean squared error\\
MSE$_{out - in}$ & MSE$_{out}$ - MSE$_{in}$ \\
$R^2_{out}$ & Out-of-sample $R^2$ \\
$R^2_{in}$ & In-sample $R^2$ \\
$R^2_{out,w}$ & Out-of-sample weighted $R^2$ (weighted by a function of dollar volume).\\
$R^2_{in,w}$ & In-sample weighted $R^2$\\
Sharpe & The Sharpe ratio \\ 
$t$-statistic & The $t$-statistic by using Newey-West estimator
\\
\hline
\end{tabular}
\label{table:para}
\end{center}
\end{table}


\begin{table}[ht]
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{minipage}{\textwidth}

\captionsetup{font=Large}
%\captionsetup{justification=centering}
\caption{Adaptive reduced rank regression on full universe}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
\hline
Test year  & N    & MSE$_{out}$ &  MSE$_{in}$ & $R^2_{out}$       & $R^2_{in}$   & $R^2_{out,w}$     &$R^2_{in,w}$   & $t$-statistic & Sharpe \\ \hline
20150701   & 2331 & 1.023  & 0.9667 & 1.802   & 330.247  & 1.2012  & 330.596  & 0.8867  & 1.3445 \\
20160701   & 2491 & 1.0205 & 0.9037 & 37.4936 & 997.3532 & 20.0247 & 868.7226 & 6.6677  & 3.2371 \\ 
20170701   & 2617 & 0.99   & 0.93   & 7.4185  & 695.0658 & 11.4901 & 736.9868 & 38.7093 & 0.9553 \\ 
all, glued & 2838 & 1.0056 & 0.905  & 18.5795 & 689.1728 & 12.1668 & 699.375  & 15.4134 & 1.6239 \\ \hline
\end{tabular}
\label{table:full_equity}
\end{minipage}}
\end{center}
\end{table}

\begin{table}[ht!]
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{minipage}{\textwidth}
\centering 
\captionsetup{font=Large}
 \captionsetup{justification=centering}
\caption{Adaptive reduced rank regression on \emph{Universe 1}}
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
\hline
Test year  & N    &  MSE$_{out}$ &  MSE$_{in}$ & $R^2_{out}$       & $R^2_{in}$   & $R^2_{out,w}$     &$R^2_{in,w}$   & $t$-statistic & Sharpe \\ \hline
20150701   & 800 & 1.0039 & 0.9738 & 99.2474 & 142.5158 & 142.8957 & 157.8843 & 5.6759 & 4.2709 \\ 
20160701   & 800 & 0.9971 & 0.9638 & 30.1577 & 178.912  & 35.018   & 206.934  & 4.3541 & 3.2096 \\ 
20170701   & 800 & 1.0123 & 0.9889 & 2.2629  & 150.4449 & 0.0266   & 134.4185 & 14.945 & 0.0517 \\ 
all, glued & 983 & 0.9935 & 1.014  & 46.3162 & 158.3772 & 70.4223  & 164.1192 & 8.3268 & 2.435  \\ \hline
\end{tabular}
\label{table:800_equity}
\end{minipage}}
\end{center}
\end{table}


\begin{table}[h!]
\begin{center}
\resizebox{0.85\textwidth}{!}{
\begin{minipage}{\textwidth}
\centering 
\captionsetup{font=Large}
 \captionsetup{justification=centering}
\caption{Summary of results for equity return forecasts}
\begin{tabular}{l|l|l|l|l|l|l|l} \hline
Model                 & MSE$_{out}$         & MSE$_{in}$         & $\text{MSE}_{out - in}$ & $R^2_{out}$(bps)        & $R^2_{in}$ (bps)           & Sharpe             & $t$-statistic     \\ \hline
$\proc{Adaptive-RRR}$, N= 983       & \textbf{0.9935} & 1.0140 & \textbf{-0.0205} & \textbf{46.3761} & 158.2564  & \textbf{2.4350} & \textbf{8.3268}  \\
Lasso              & 1.1158 & 0.3953 & 0.7205 & 6.6049  & 7147.0116 & 2.1462 & 0.0601  \\ 
Ridge              & 1.2158 & 0.1667 & 1.0491 & 9.8596  & 8511.9076 & 0.6603 & -0.0497 \\ 
Reduced ridge & 1.0900 & 0.8687 & 0.2213 & 13.0321 & 1555.5136 & 0.3065 & -0.3275 \\ 
RRR &  1.2200 & 0.5867 & 0.6332 & 7.0830 & 4121.2548 & 0.3647 & -0.6626\\ 
Nuclear norm &  1.2995 & 0.12078 & 1.1787 & 4.7297 & 8789.0625 & 0.6710 & 0.2340\\

\hline
$\proc{Adaptive-RRR}$, N= 2838      & \textbf{1.0056} & 0.9050 & \textbf{0.1006} & \textbf{18.5761} & 689.0625  & \textbf{1.6239} & \textbf{15.4134}\\ 
Lasso              & 1.0625 & 0.5286 & 0.5339 & 1.1236  & 6029.5225 & 0.5954 & 0.0179  \\ 
Ridge              & 1.0289 & 0.6741 & 0.3548 & 0.2116  & 5342.1481 & 0.5739 & 0.0670  \\ 
Reduced ridge & 1.9722 & 0.7373 & 1.2349 & 1.0816  & 2416.7056 & 1.5482 & 0.0619  \\ 
RRR & 1.0873 & 0.61376 & 0.4735 & 4.5795 & 3844.124 & -0.477 & 0.6399\\
Nuclear norm & 1.1086 & 0.15346 & 0.9551 & 2.2097 & 8461.2402 & -0.3698 & -0.8986 \\
\hline
\end{tabular}
\label{table:full_compare}
\end{minipage}}
\end{center}
\end{table}
\myparab{Characteristics of the portfolio.} We next describe the characteristics of the portfolio constructed by using our model's forecast. See Table~\ref{table:full_equity},~\ref{table:800_equity} for the breakdown of returns. Note that we also report weighted correlation. The weights are determined by the historical dollar volume of the asset. This statistics is useful because the positions taken by the optimizer are sensitive to the historical dollar volume. Figure.~\ref{fig:preY_statisticaa}(a) shows the distribution of the standard deviation of our returns at daily granularity from the forecast in Table~\ref{table:800_equity}. This measures the ``aggressiveness'' of our forecasts. When the forecasts have high standard deviation, they push the optimizer to take larger positions. We note that while the standard deviations are time-varying, our forecasts rarely bet more than $60bps$. This is an evidence that the forecast picks up the market structure from training.  Figure.~\ref{fig:preY_statisticaa}(b) plots the distribution of returns from our portfolio at daily granularity. We see that this is a ``statistical betting:'' a considerable fraction of our betting loses money. However, if we bet frequently enough, our portfolio is still able to maintain a high Sharpe. We remark that the performance may reduce when we consider the transaction costs.

\myparab{Results.} Our data span May 1, 2011 through July 30, 2018. We report the forecasting power and portfolio return for \emph{out-of-sample} periods. 
Each training period consists of approximately 720 observations (one observation is a $(\mx_t, \mr_t)$ pair). Each forecasting period consists of approximately 240 observations. Table ~\ref{table:full_equity} and~\ref{table:800_equity} report the full results of the two universes.
%and top $20\%$ (in terms of dollar volume) from 300 index. 
See Table~\ref{table:para} for detailed  descriptions of data columns.



\mypara{Obs 1. High signal to noise.} For all the methods we examined, the out-of-sample $R^2$ are all close to 0.
%normalized MSE's (normalized by standard deviation of the responses) are all close to 1 (0.95 to $> 1$). This phenomenon is ubiquitous across all major markets.      

\mypara{Obs 2. $\proc{Adaptive-RRR}$ has the highest forecasting power ($R^2$).} Among all models, our method has the highest out-of-sample $R^2$. An interesting property here is that Reduced ridge has considerably worse performance, suggesting that our model appears to be more robust in financial datasets.  

\mypara{Obs 3. In-sample and out-of-sample gap.} Our method has the \emph{worst} in-sample $R^2$ but achieves the best out-of-sample $R^2$ and the \emph{smallest gap} between in-sample and out-of-sample performance (in $R^2$). MSE shows a similar pattern. This suggests that our model is better at avoiding spurious signals, and thus achieves our major design goal.  

==> notation_table.tex <==
\section{Table of Notation}

\begin{tabular}{ll}
	$C^*$ & $C^* = \E[\vx\vx^\top]$ \\
	$U^*, \Sigma^*, V^*$ & Given by the SVD of $C^* = U^*\Sigma^* V^*$ \\
	$\Lambda^*$ & $(\Sigma^*)^\frac{1}{2}$ \\
	$N$ &  $N = M V^* (\Lambda^*)^\frac{1}{2}$\\
\end{tabular}

